Self-distilled Dynamic Fusion Network for Language-based Fashion Retrieval

In the domain of language-based fashion image retrieval, pinpointing the desired fashion item using both a reference image and its accompanying textual description is an intriguing challenge. Existing approaches lean heavily on static fusion techniques, intertwining image and text. Despite their commendable advancements, these approaches are still limited by a deficiency in flexibility. In response, we propose a Self-distilled Dynamic Fusion Network to compose the multi-granularity features dynamically by considering the consistency of routing path and modality-specific information simultaneously. Two new modules are included in our proposed method: (1) Dynamic Fusion Network with Modality Specific Routers. The dynamic network enables a flexible determination of the routing for each reference image and modification text, taking into account their distinct semantics and distributions. (2) Self Path Distillation Loss. A stable path decision for queries benefits the optimization of feature extraction as well as routing, and we approach this by progressively refine the path decision with previous path information. Extensive experiments demonstrate the effectiveness of our proposed model compared to existing methods.

==> subsection/related.tex <==
\section{Related Work}

\subsection{Composed Image Retrieval}
The composed image retrieval (CIR) was first proposed by ~\cite{Vo2018ComposingTA} and has gained significant attention in recent years. Compared to conventional retrieval patterns that primarily focus on image-image retrieval~\cite{Noh_Araujo_Sim_Weyand_Han_2017,Sharma_Vishvakarma_2019} and text-image retrieval~\cite{Zhang_Lei_Zhang_Li_2020,Xu_Wang_Yang_Zuo_Shen_Shen_2020}, composed image retrieval allows users to express their search intentions and interact with the retrieval system, resulting in a greater possibility of retrieving the desired item. To tackle this task, recent works~\cite{Anwaar_composeae_2020,Lee_cosmo_2021,Shin_rtic_2021,Delmas2022ARTEMISAR,Kim_dcnet_2022,Dodds_maaf_2020} have devised various image-text composition modules for retrieval. TIRG~\cite{Vo2018ComposingTA}utilizes gating and residual mechanism to compose the reference image and the modification text. ARTEMIS~\cite{Delmas2022ARTEMISAR} first divides the task into image-image retrieval and text-image retrieval. Subsequently, the results from these two groups are combined to generate the final predictions. VAL~\cite{Chen_val_2020} conducts 
fusion operation on features extracted from different stages of the image encoder and performs hierarchical feature matching to obtain the final results. CosMo~\cite{Lee_cosmo_2021} employs a content modulator and a style transformer to disentangle the image-text fusion process into two consecutive procedures. CLVC-Net ~\cite{Wen_clvcnet_2021} seamlessly unifies the fine-grained local-wise composition and the coarse-grained global-wise composition, taking into account both local and global information. ComqueryFormer~\cite{Xu_comqueryformer_2023} utilizes a uniform transformer architecture to perform feature extraction and image-text composition, thereby mitigating the architectural discrepancies. 

Despite the remarkable advancements achieved by these methods, their approaches of applying identical fusion operation to all diverse input image-text pairs restrict the flexibility and generalization capability of the model. Therefore, our objective is to maximize the level of flexibility and diversity of image-text fusion modules to offer more comprehensive modality interactions through the dynamic fusion network.

\subsection{Dynamic Network}
In the field of computer vision, numerous deep models~\cite{Krizhevsky_alexnet_2017,Vaswani_trans_2017} have achieved remarkable achievements owing to their intricate and sophisticated architectures. Recent development in neural architecture search (NAS)~\cite{Liu_darts_2018,Chen_sdrats_2020,Yu_MMNas_2020} presents a multitude of possibilities for model architecture design. However, one common characteristic among these methods is the utilization of a static model during the inference stage. Dynamic networks, in contrast to static models, possess the ability to adjust network structures based on input during inference. Cai~\textit{et al.}~\cite{Cai_drnet_2021} propose DRNet, an efficient and flexible backbone network that can dynamically produce a tailored architecture for each input during inference. Xue~\textit{et al.}~\cite{Xue2022DynamicMF} propose a dynamic multimodal fusion network with hard gates to determine the appropriate fusion operations to employ. Due to the use of a hard gate, only the fusion module with the largest weight will be chosen, and those with lower weights will be discarded, leading to the loss of information. Qu~\textit{et al.}~\cite{Qu_DIMe_2021} first introduced a dynamic modality interaction model towards image-text retrieval, offering a novel approach to tackle the main challenges of intra-modal reasoning and inter-modal alignment in conventional image-text retrieval tasks.
 

